Learning Patterns and Abstractions from Perceptual Sequences

Cognition swiftly breaks high-dimensional sensory streams into familiar parts and uncovers their relations. Why do structures emerge, and how do they enable learning, generalization, and prediction? What computational principles underlie this core aspect of perception and intelligence? A sensory stream, simplified, is a one-dimensional sequence. In learning such sequences, we naturally segment them into parts -- a process known as chunking. In the first project, I investigated factors influencing chunking in a serial reaction time task and showed that humans adapt to underlying chunks while balancing speed and accuracy. Building on this, I developed models that learn chunks and parse sequences chunk by chunk. Normatively, I proposed chunking as a rational strategy for discovering recurring patterns and nested hierarchies, enabling efficient sequence factorization. Learned chunks serve as reusable primitives for transfer, composition, and mental simulation -- letting the model compose the new from the known. I demonstrated this model's ability to learn hierarchies in single and multi-dimensional sequences and highlighted its utility for unsupervised pattern discovery. The second part moves from concrete to abstract sequences. I taxonomized abstract motifs and examined their role in sequence memory. Behavioral evidence suggests that humans exploit pattern redundancies for compression and transfer. I proposed a non-parametric hierarchical variable model that learns both chunks and abstract variables, uncovering invariant symbolic patterns. I showed its similarity to human learning and compared it to large language models. Taken together, this thesis suggests that chunking and abstraction as simple computational principles enable structured knowledge acquisition in hierarchically organized sequences, from simple to complex, concrete to abstract.

==> content/colophon.tex <==
% !TEX root = ../thesis-example.tex
%
\pagestyle{empty}
\hfill
\vfill
\pdfbookmark[0]{Colophon}{Colophon}
\section*{Colophon}

This thesis was typeset with \LaTeXe.
It uses the \textit{Clean Thesis} style developed by
The design of the \textit{Clean Thesis} style is inspired by user guide documents from Apple Inc.

% Download the \textit{Clean Thesis} style at \url{http://cleanthesis.der-ric.de/}.


==> content/dump.tex <==
\chapter{Introduction}
\label{sec:intro}


Our sensory input contains this vast intrinsic complexity and dimension that any attempt at summarizing experience with an artificial articulation of pronunciation or representing it from some artificially composed symbols will inevitably results in a significant loss of information. Echoing this sentiment, Lao Tzu, the founder of Taoism in ancient Chinese philosophy, inaugurated the seminal Taoist text, the "Tao Te Ching," with an assertion: if one claims to articulate the Dao (the fundamental principle underlying the natural order of the universe), then what is being described is not the true process of the Dao ---- underscores the limitation of language and symbols in capturing the nuance of the universe.

% aristotle studied cateogories 
During the same era as Lao Tzu, on the distant shores of Ancient Greece, Aristotle was thinking about a related question: What is the nature of knowledge, and what are the essential components of logical deduction that empower us to reason and apply logical principles to deduce new knowledge?

As the cornerstone in the development of philosophical thought he was laying the groundwork for the formal study of logic and reasoning. Namely, we can reason about unexperienced knowledge based on logical deduction rules. Such as knowing that Socrates is a human, and humans are mortal, would enable us to deduce that Socrates is mortal. To form a such logical syllogism, Aristotle noted that it is necessary to form the initial establishment of predicates for logical deduction. These predicates typically arise from the categories we discern in our perception: distinctions such as height, size, the identification of Socrates, the classification of beings as human, and an understanding of mortality. 

Aristotle believed a methodical examination of these categories, which form the foundational elements of logical propositions, was critical.
He embarked on creating a detailed framework of categories, including identifying objects and perceiving their physical relationships to one another—whether they be large or small, near or far—along with causality and other relational concepts.
Aristotle underscored that these categories not only serve as the underpinnings of logical deduction and induction but also facilitate the process of deductive reasoning. 
This pioneering exploration by Aristotle essentially marked the formulation of reasoning as a structured process, treating discrete representations of objects as subjects for computational analysis. 
%he also realized the importance of ideas and cateogories as an ingredient 


% summary:
Before psychology, cognitive science, and neuroscience, philosophers noticed a common theme in perception: despite the inherently sequential, temporal, multidimensional, chaotic, and the ephemeral nature of existential experience, humans possess the remarkable ability to distill this complexity into the conception of discrete objects and to understand the dynamics of their interactions and relationships. We grant names to objects and ideas and communicate with each other to bridge the perception of the universe of two beings. We argue with each other to deduce to an agreed-upon set of beliefs of how the world functions, which comes to their existence manifested in a collective knowledge system, which updates with scientific advances and some of them forgotten by memory. Identifying the discrete symbolic content of perception simplifies record and communication. It enables logical deduction, which lays the foundation of the subsequent work on scientific thought and the development of scientific theories in the upcoming centuries. How patterns emerge from observation seems to be the central theme that pushed the evolution of cognition and intelligence. 


%
Piaget has famously posited a developmental trajectory of world understanding. 
Starting with the initial, booming, buzzling confusion, the infant does not differentiate a dissociation between the external and the internal world, rather, perceptions consists of mobile and plastic sensations. Amongst such chaos, the second stage of understanding is marked by an aggregation of groups of sensations. The grouping of sensory stimuli that occur similarly in perceptual space-time assist the child to identify object permanence, and differentiate subjective groups such as categories of emotion to objective groups such as objects. Concurrently, the child learn to identify causal relations, and realize that the self can be the cause of consequences in the world, which triggers the third stage of development: the evolution of schemata, which composes the logical concepts and relations sufficient to become a component of mental deduction. According to Piaget, our understanding of reality is constructed through developmental stages. Developing over time, we gradually organize and interpret sensory information into coherent experiences. 
\subsection{empiricists}
During the Enlightenment, British empiricists emphasized that all knowledge derives from empirical observations. John Locke gave an account of how ideas derive from experience from his tabula rasa theory:  newborn human babies do not process the objects and relations as characterized by Aristotle. Instead, they process a blank (\textit{tabula rasa}) state of mind. However, the human mind is equipped with faculties that enable it to derive ideas from perception and acquire the relations amongst the ideas, amongst which include memory. (Locke, the limits of human understanding, Book II).
David Hume introduced the minimal amount of machinery that he thought would warrant an operation of a mind — all derived from experience. He noticed that perception comes first to the mind as vivid ‘impressions’; only later do we develop ‘ideas’, which are much more abstract and less lively compared to impressions, which emerge only later after the impression has been familiarized with memory. All human imagination is essentially a composition of existing ideas derived from perception and impression. Hence, a naturally blind man cannot form the idea of color in his imagination because he has not formed any impressions associated with color before. When imagining an elephant with a pair of wings, we are composing the idea of an elephant with the idea of wings, acquired from separated impressions derived from perceptions. Hume also noted that ideas interact in a finite number of ways: 1)Resemblance. 2) Identity. 3) Space and time.4) Quantity, or number. 5) Degrees. 6) Contrariety. 7) Cause and Effect. For example, after observing one event succeeding another, the ideas then join together to form causal relationships. Whilst man is thinking, ideas emerge sequentially; all arise from the perceptual experience of observing and interacting with the world. 









%\subsection{Factorization relates to learning a causal structure}
% symbols are related to the parts in causal graphical models, which is another branch that tries to extract interpretable representation as good models for data. 
%The literature of probabilistic graphical models and causal inference provided a proposal for the inference of Probabilistic entities based on observation. Usually, the entities in the world are described as a set of random variables. The dependencies of some variables on others are described as the conditional probability of a variable conditioned on a set of other variables. 
% yet this branch is also still researching the origin of structures, i.e., where do causal graphical structure come from

%\subsection{Structured symbolic models have proven to be good cognitive models of human behavior via Bayesian Inference}

% bayesian inference 
%One rational framework of learning represented in the symbolic form is the Bayesian cognitive model. Bayesian cognitive models define probabilities over structured symbolic forms of knowledge representation, such as graphs, grammar, predicate logic, and others. Usually, these models assume structured symbolic forms to factorize data, manifested in some causal graphical models. 

%Learning in this domain becomes inferring the most likely hypothesis amongst the structured representations given observation. Hypothesis about the structure of the world is encoded through a hypothesis space with latent variables. Conditioning on the observation data, Bayes rule updates the beliefs about the hypothesis through 
%$P(h|d) = p(d|h)P(h)/sum_{h’}P(d|h’)P(h’) \prop P(d|h)P(h)$. $p(d|h)$ is the likelihood of data under the hypothesis h, and $P(h)$ is the prior probability integrating the background knowledge. For example, When a friend is seen as sneezing, it can be caused by a cold or heartburn, but a cold is more likely given the higher likelihood of a cold happening than heartburn, and thereby, one can arrive at the most rational estimation of the possible cause of sickness. Learning then translates to an update on the parameters that update from prior distribution to posterior distribution given observation data. Sometimes, the hypothesis can also not just be one latent variable, but also programs. 

%Hierarchical Bayesian modeling takes Bayesian modeling to a higher level of sophistication. The levels of hierarchy represent classes of hypotheses and, sometimes, schemas. On an abstract level, the hypothesis can be a network-structured representation or a tree-structured representation; lower in the hierarchy can be the specifics of the network and tree structure. In this case, the model searches through a combination of programs that explain the observed data with the most likelihood. Update beliefs about latent variables of the generative model. The nonparametric variation of the Bayesian model offers the flexibility also to learn a variable number of states or structures used to characterize data. But in this case, the modeler still would need to define the structure of the causal model. [TODO: insert nonparamettric discussion]



% [maybe go to discussion]\cite{abel_near_nodate} proposes using state abstraction to alleviate the combinatorial explosion problem that plagues planning in reinforcement learning algorithms. In their framework, the state space of a ground MDP is mapped to that of an abstract MDP, which treats nearly identical states as the same. They derived guarantees of theoretical optimal behavior with the abstract MDP. They also show that abstraction provides the benefit of task complexity reduction and bounded loss of optimality. 


% stay in a non-probabilistic regime, probability is an add-on of the future
Hence towards answering the above two questions, we do not develop algorithm that integrate probability. While probabilistic algorithms are useful to characterize a distribution of human behavior. Because the integration of probability into a noisy algorithm will only hinder a good understanding of it. Probability is an add-on, but it creates unnecessary burden as the first step to tackle a question.  We reserve this aspect of work to the future and focus on simplifying the understanding for now.  




% \subsection{Neural Implementable}
% % neural implementable. 
% On the other hand, we would like to reduce the search range of cognitive models within those that can naturally emerge from the neural activities in the brain. As it would not make too much sense to build models that are hard or implausibly implemented by the biological organism that we are endowed with.  

% %THe thesis proposes algorithms that employes simple cognitive principles can give rise to complex structures of representation. Simple to the extend to be easily computed by our biologically endowed neural substrates. 




%It has been known that neurons adapt to repeated occurrence in stimuli. It has been long used as a technique in fMRI studies to turn off neural activities by showing repetitions of the identical stimulus. It is very possible that learning to predict and adapt representations from repeated stimuli in sequences are the most fundamental task facing biological neural networks even of the simplest kind.


%When a male fruitfly courts, he orients towards the female, tap with forelegs, extend a wing, and vibrates to sing. From individual muscular contractions to a complete sequence of the courtship process, One can predict short-term animal behavior with fine-grained behavioral representation and longer-term behavior with coarser representations \cite{Berman2016}. Behaviors within each repertoire tend to happen rather independently of behavior that belongs to other modules. These behavioral modules are expressed in predictable sequences over time and organized hierarchically at multiple timescales. 



%Other models of chunk proposal are neural network based \cite{french_tracx_2011, cleeremans_finite_1989}. TRACX uses a three-layer feedforward backpropagation autoassociator and adapts the autoassociator’s weights to the difference between its prediction and actual sequential units when this difference exceeds a pre-defined threshold. \cite{Wang2017APlasticity} trained a self-organized recurrent spiking neural network with spike-timing-dependent plasticity and homeostatic plasticity on sequences. The model was shown to reproduce several sequence learning effects .

%The two model types mentioned above are process models. In contrast to process models stand normative statistical models, which model the ideal observers’ behavior. This approach includes variants of the Bayesian ideal observer framework \cite{Goldwater2009}. Given a linguistic corpus, these models find a segmentation with the highest probability that contains relatively few word types, exploiting the minimal description length principle. These models are also rational because their inference is evaluated on observational instances. They provide accounts for high-level computation required for chunk learning. As normative and process models rely on different principles, they are usually not compared against each other.

% chunks maybe a strategy to speed up learning 


The storage problem is strange. For the symbols that humans have seen, there is potentially infinitely amount of storage to record what we have seen in the past.  Similarly, there is potentially an infinite amount of storage to store how often one thing is followed by another thing in long term memory.  However, there is a finite amount of capacity that we processes short term memory into long term memory. 
If we assume that the brain processes information in an optimal manner, that is, retrieval time and difficulty is directly related to how often this stimuli is going to be used by the brain, then we can assume that storage in the brain is related to the entropy of a certain piece of information. 




\section{What goes inside the magical number 7?}
Miller famously report that our short-term memory is limited to hold 4 to 7 chunks. To this end, separate sequential elements merge into one cognitive entity. This cognitive entity is then recalled and identified as a whole \cite{Mathy2012WhatsMemoryb}: a phenomenon known as \emph{chunking} \cite{Lashley1951TheBehavior,Gobet2001ChunkingLearning}. 

% Cognitive scientists have discovered that chunks, instead of sequential items, are what goes inside the the magical number 7
When humans are instructed to remember a long sequence, researchers have noticed that we tend to break a sequence into several parts. To give an illustration, upon reading DFJKJKJKDFDFJK, you will likely group DFs and JKs as a unit --- an instinctive tendency to break a sequence into segments of familiar parts. Once a chunk has been learned, it is memorized, identified, and parsed as a whole \cite{Egan1979ChunkingDrawings, Lashley1951TheBehavior, Verwey1996BufferKeypressing}.

While chunking may not be very explicitly implied in serial sequence learning tasks, the terminology actually comes from memory experiments. 
% Cognitive scientists have discovered that chunks, instead of sequential items, are what goes inside the the magical number 7
When humans are instructed to remember a long sequence, researchers have noticed that we tend to break a sequence into several parts. In our short term memory, people can on average hold from 4 to 7 chunks. This implies that \cite{Miller1956TheInformation}longer chunks helps us to remember longer sequences. Imagine having to remember the sequence ``052917080461''. Taken on its own, this sequence might be difficult to remember. However, knowing that it contains both John F. Kennedy's and Barack Obama's date of birth will likely simplify remembering the sequence. Even small babies learn to segment language. Chunking allows subjects to store a longer sequence within a limited span of their short-term memory, and functions as a basic unit of cognitive processing. 


\section{Literature}
fmri data set watching movies 
 relationship between perceived event boundaries and neural pattern shifts. By applying an innovative analysis to a large, publicly available dataset, they observe evidence of different timescales of neural state shifts that correspond with perceived event bounds
 \cite{geerligs2022}


\item Irregularity Detection. Participants who have learned a better internal chunking model of the sequence are able to detecting abnormality in the generating sequence much faster than those who hasn't. Abnormality refers to mutated observations that is inconsistent with the generative model of the sequence used to for training subjects. This is because compositional chunks helps to scale up subject's predictive power, and in turn, enables them to allocate attention to the most surprising observation violating their internal model. 


When there is a sentence composition that does not fit into our expectation of a grammatical structure, it triggers an inherent discomfort to be acutely aware of reading something violating the regularities that we expect.

% Beyond comprehending allegories, knowing the solution of one problem helps people to come up with ideas to solve another problem. Druncker \cite{duncker_problem-solving_1945} famously tested the facilitation of metaphor in problem solving by presenting participants this problem:

% Imagine that you are a doctor facing a patient with a malignant tumor in his stomach. There is a ray that can be used to destroy the tumor. If you inject the ray all at once with sufficiently high intensity, it destroys healthy tissue. However, if you lower the ray intensities, it destroys neither the tumor nor the healthy tissue. 

% Participants are then asked to describe a strategy to destroy the tumor while maintaining the healthy tissue intact. 

% Afterwards, participants are presented with another scenario:
% A general is tasked with capturing a fortress. Many roads radiate outward from the fortress. All roads are mined. Small groups of men can pass over the roads, but a large force will detonate the mines and decimate the army. The general came up with a solution: divide the army into small groups, send each group on a different road, and have the groups converge simultaneously on the fortress. 

% Drunker found that after learning about the general's solution, participants can quickly and easily come up with the solution facing the tumor problem. Having seen the solution to the general's problem and the resemblances between the general's and the doctor's problem dramatically helped participants immediately come up with the solution to a problem in a completely different scenario.

% The examples in reasoning and problem solving points to our inherent tendency to discover motifs between distinct instance. What is this tendency of the cognitive system to the common amongst the distinct? And what is the influence of such ability in our memory and generalization behavior? 


\subsection{Chunking models, and markov models with memory}
Even in a sequence with just a few chunks, it translates to a very long sequence when it is expressed in n-gram. 

Although we tried to study this question, we never found a clean and nice expression for how to translate the chunk structure into the memory of the ngram model. 

I hope future work can come up with a nice way of describing the relationship between chunking and n-gram models that learns the conditional probability given a particular length of observation history. 


Human acquisition of problem solutions is not in a graded fashion but rather contains this step-wise characteristic of realizing a solution all of a sudden. We hypothesize that the aha moment may stem from identifying an analogical structure from a previously learned concept to the current problem. The search process of finding the previously learned concept to explain the current observation will yield no reward or insight until the search process arrives at the previously learned conceptual structure, thereby enable a step-wise advancement of problem solution when the relevant concept has been identified.  The progressive construction of knowledge would predict that the aha moment would process to be more efficient from a source problem to a target problem with an increasing amount of practice. 

When stimuli of the same category or concept duplicates, such as the experience of petting a neighbor's dog and observing cars on the street, occur at sporadic time points in our lives, the imprint of those perceptual stimuli on the memory gradually supports the emergence of concepts. Thereby can we establish the idea of 'zoey' as being the neighbour's dog, recognize and recall the interaction with 'zoey' when her name as been mentioned, even though 'zoey' by itself is only a combination of two, otherwise, meaningless syllables. But after a child has interacted with 'Zoey,' the written symbols or the physical pronunciation of the two syllables is able to instantiate the fond collections of memories from the child of the interactions with the neighbor's dog. 

The identification of repeated patterns or symbols in perception is a main ingredient that also constitutes the memory construction process, equipping us with the ability to memorize an event even after years of its occurrence, helping us to arrive at a constitution of our personal, bibliographical timeline, to jump back in time via reminiscence, and to re-experience in light of later-acquired knowledge. 


%%%%%%%%%%%%%%%%%%%%%%% ARXIV


 % candidate quotes 


 \cleanchapterquote{The propose of science is to find meaningful simplicity in the midst of disorderly complexity.}{Herbert Simon}{}

 \cleanchapterquote{Der Mensch ist ein Seil, geknüpft zwischen Tier und Übermensch – ein Seil über einem Abgrunde.}{Friedrich Nietzsche (1844 - 1900)}{}


 \cleanchapterquote{“Reality is merely an illusion, albeit a very persistent one.”}{Albert Einstein}{Physicist}

“A human being is a part of the whole called by us universe, a part limited in time and space. He experiences himself, his thoughts and feeling as something separated from the rest, a kind of optical delusion of his consciousness. This delusion is a kind of prison for us, restricting us to our personal desires and to affection for a few persons nearest to us. Our task must be to free ourselves from this prison by widening our circle of compassion to embrace all living creatures and the whole of nature in its beauty.”
― Albert Einstein

“The world as we have created it is a process of our thinking. It cannot be changed without changing our thinking.”
― Albert Einstein


"You must be shapeless, formless, like water. When you pour water in a cup, it becomes the cup. When you pour water in a bottle, it becomes the bottle. When you pour water in a teapot, it becomes the teapot. Water can drip and it can crash. Become like water, my friend." — Bruce Lee

“I also consider that plain living is good for everybody, physically and mentally.”
― Albert Einstein, The World As I See It

“And those who were seen dancing were thought to be insane by those who could not hear the music.”
― Friedrich Nietzsche

“When someone seeks," said Siddhartha, "then it easily happens that his eyes see only the thing that he seeks, and he is able to find nothing, to take in nothing because he always thinks only about the thing he is seeking, because he has one goal, because he is obsessed with his goal. Seeking means: having a goal. But finding means: being free, being open, having no goal.” 
― Herman Hesse, Siddhartha


“That is where my dearest and brightest dreams have ranged — to hear for the duration of a heartbeat the universe and the totality of life in its mysterious, innate harmony.” 
― Hermann Hesse, Gertrude


“There is no escape. You can't be a vagabond and an artist and still be a solid citizen, a wholesome, upstanding man. You want to get drunk, so you have to accept the hangover. You say yes to the sunlight and pure fantasies, so you have to say yes to the filth and the nausea. Everything is within you, gold and mud, happiness and pain, the laughter of childhood and the apprehension of death. Say yes to everything, shirk nothing. Don't try to lie to yourself. You are not a solid citizen. You are not a Greek. You are not harmonious, or the master of yourself. You are a bird in the storm. Let it storm! Let it drive you! How much have you lied! A thousand times, even in your poems and books, you have played the harmonious man, the wise man, the happy, the enlightened man. In the same way, men attacking in war have played heroes, while their bowels twitched. My God, what a poor ape, what a fencer in the mirror man is- particularly the artist- particularly myself!” 
― Hermann Hesse


“Every man is more than just himself; he also represents the unique, the very special and always significant and remarkable point at which the world's phenomena intersect, only once in this way, and never again. That is why every man's story is important, eternal, sacred; that is why every man, as long as he lives and fulfills the will of nature, is wondrous, and worthy of consideration. In each individual the spirit has become flesh, in each man the creation suffers, within each one a redeemer is nailed to the cross.” 
― Hermann Hesse , Demian. Die Geschichte von Emil Sinclairs Jugend



“No one is willing to believe that adults too, like children, wander about this earth in a daze and, like children, do not know where they come from or where they are going, act as rarely as they do according to genuine motives, and are as thoroughly governed as they are by biscuits and cake and the rod.” 
― Johann Wolfgang von Goethe, The Sorrows of Young Werther



==> content/ex-chapter-futurework.tex <==
% !TEX root = ../thesis-example.tex
%
\chapter{Future Work}

\label{sec:system}

% something that integrates interpretable with the uninterpretable % something uplifting 
% something that marks an end and a new beginning 
% \cleanchapterquote{placeholder}{}{}
Future work can expand this thesis in three directions. 
One direction is understanding and interpreting human and animal behavior and the neural computations that give rise to learning hierarchically structured sequences. 
The second direction is to use chunking as a tool of interpretation to understand other intelligent agents learning from structured input statistics.
The third direction is to scale the model up and express learning high-dimensional structure in clearly articulated ways. The above three directions are described in the following three sections. 


\section{Uncovering the orchestration of neural activities underlying behavioral sequences}
% evidence about the chunks in animal behavior and behavioral hierarchies. 

% since we are brains studying brains, understanding is structured in brain-comprehensive ways 

% brains studying artificial brains 

%Both artificial and biological agents aim to extract disentangled representations from naturalistic data, which contains a hierarchical structure. 
% one can engineer the 'optimal' curriculum according to some physiological property of the animal/human
% [ ] explain better 
\subsection{Hierarchies in behavioral sequences}
Models that learn recurring patterns in data can be extended to discover the structure of animal movements. Hierarchy has been hypothesized to be the language of behavior: from nematodes to fruitflies to mice and to humans, animals combine simple motor primitive into more complex behavioral repertoire \cite{Baerends1976TheFO, Tinbergen1951, Berman2016}. Caenorhabditis elegans roams around by bending its body on a scale of sub-seconds; the combination of several bends then becomes a basic crawling movement. Different combinations of crawling constitute the worm's exploration and quiescence behavior, which repeat and reoccur depending on the state of the environment \cite{KAPLAN2020562}. It is also known that mice possess basic movement modules such as running, rearing, and grooming. They flexibly place the movement modules into sequences of behaviors. Instead of generating an entirely new set of behaviors, the movement modules tend to be reused and become a basis of modification when new stimuli are introduced in the environment, such as when the mouse smells fox odor \cite{WILTSCHKO20151121}.  

In these behavioral domains, models such as HCM can be adapted to extract the minimal set of stereotyped animal movement motifs, thereby allowing the annotation of animal movements via identifying individual motifs from a movement dictionary. Annotating behavior in this way helps us study the composition of animal movements. It helps with understanding behavioral questions such as the organizational structure of behavioral motifs, the difference between individual animals, how animals chain movement motifs to compose complex sequences, the relation between movement motif and the energetical and psychological state of the animal, and the consequences of interruption and novel stimuli on the motif structures during execution.  

%Moreover, animals compose their behaviors from a context-specific set of repeatedly-used stereotyped movement motifs. 

%Close perceptual components are grouped into one part and considered as a whole. In sequence learning, close perceptual components are consecutive observations. In motion, structural perception, close perceptual components are grouped together as a whole. 



\subsection{Uncovering robust firing activities amongst biological neurons}
% [ ] sequences % use Hcm to discover sequences
Going towards a neural implementation level, future work could extend this model to study the neural basis that give rise to  movement motifs in animals. 
%, and has been hypothesized to be governed by some universal neural coding principle that relates to the temporal clustering of hierarchies in the motor cortex.
On a neural level, transient sequential neural firing activities have been robustly observed across animal species and multiple brain areas. These sequential firing patterns have been associated with spatial navigation, learning, sleep \cite{Lee2002,Wilson1994}, and planning \cite{Diba2007}. For example, when a rodent navigates around a familiar environment, synchronous firing of inter-correlated neural subpopulations was observed in hippocampal pyramidal cells in the medial temporal lobe (MTL) \cite{vaz_replay_2020}.
The same neural firing sequence replays when the rodent is awake and sleeping \cite{Foster2006}; also, when the animal makes decisions at a crossroad, the preplay of neural sequences corresponding to the rodent's subsequent action can be observed and reliably predict the rodent's choice. 

% importances of sequences in neural activities 
In primates, neurons in the prefrontal cortex correspond to encoding the switching of abstract rules \cite{wallis_single_2001}. In humans, it has been similarly suggested that sequences of neural activity patterns underlie cognitive operations, including memory retrieval,  consolidation, planning \cite{vaz_replay_2020}, and creative thought \cite{buzsaki_hippocampal_2015, joo_hippocampal_2018, buzsaki2010neural}. Experiments suggested that episodic memory is encoded by specific sequences of neural activity, and memory recall involves reinstating this temporal order of activity \cite{vaz_replay_2020}. A robust retrieval of neural sequences related to the first experience in memory is associated with the successful retrieval of individual episodic memory \cite{Gelbard-Sagiv2008,Carr2011,Eichenbaum2013}. In future work, models such as hierarchical chunking or variable learning models can be adapted to discover the recurring succession of transient neural firing patterns amongst biological neural activities. These sequences of neural firing activities can be used as units to parse and interpret neural activity sequences. %Chunking can be a method to extract robustly recurring sequential firing patterns in biological neural population activities.

\subsection{Studying the relation between neural hierarchies, reuse, and compositionality in biological neural populations}

% [ ] hierarchies  
% neural activities contain inherent structure within
It is not just repeating sequences that are represented robustly as sequences of firing patterns in the brain; experiments also discovered that biological neural activities contain a hierarchically nested structure, oftentimes reflecting the nested structure in input sequential stimuli. In the human brain, studies have discovered the existence of neural populations sensitive to the chunk boundaries. Some neural oscillation frequencies reflect the nested structure in linguistic sequences on an organization level of syllables, words, and phrases \cite{kaufeld_linguistic_2020}, resonating with our discovery of rich nested structures of activity patterns in fMRI data \cite{wu_learning_2022}. In future work, this work can be adapted to identifying groups of coordinating brain regions corresponding to observed structural and functional connectivity in the literature on a finer scale.

People have hypothesized about the rationality of hierarchical organization structure in the neural system. 
Supposedly, the hierarchical structure of an organization makes complex behavioral programs easier to code by the neural system \cite{KAPLAN2020562, Berman2016}. Since neural activities change at a slow time scale and are usually not easily malleable, composing existing neural computations that drive behavior primitives and reusing existing neural modules breaks complex tasks simpler for our biological neural substrate. Because of this reason, it has been hypothesized that the neural cell assemblies are organized in a hierarchical manner, and the structure of the hierarchy is determined by synaptic weight modifications \cite{Bressler2006, Harris2005,Luczak2015}. Future work may look into the neural basis of synchronous correlated sequences of neural firing activities and may provide some justifications and explanations for why chunking is profoundly observed in cognition. 
%[ ] say how this model can be applied to this area 

%Applying chunk learning principles to biologically realistic artificial neural circuits [parallel, efficient, ]
In our previous work, we  also tested the applicability of chunk learning on biologically realistic neural circuits. In mixed-signal neuromorphic hardware that emulates the firing activities of simple biological neural circuits, we demonstrated a group of spiking neurons with biologically plausible principles of synaptic plasticity and homeostasis that can efficiently parse chunks and learn nested patterns from sequences. This work suggests that the parallel computation of the neural system is naturally efficient in retrieving a successive activation of neural sequences upon. The project demonstrated the computational advantages that neural circuits hold to learn nested hierarchical sequences and parse them in a power-efficient way \cite{schreiber2023biologicallyplausible}. 

Apart from identifying repeating neural firing sequences, more pressing still will be the use of our model to study the relations amongst these neural computation primitives. 
In future work, a structured understanding of robust repeated sequences of neural activities can be a lens for comprehending the interactions amongst neural populations that represent sequential primitives. This algorithm can be used to study the neural implementations of compositionality on an implementation level, such as how primitives of activation sequences arise from neural populations during training and how the robust neural firing sequences can be reused and re-proposed to conduct transfer tasks in a new environment, or to be chained together to form more complex action sequences, and what sort of information is being ignored and abstracted in neural computation. 


% [ ] maybe some plots to illustrate this point 

% [ ] figure: of hierarchical organization of animal behavior 

% % reuse can be also very important for biological neuronal populations,
% Because the activity pattern that a neural population can generate can be very constrained. And reassociating the pre-exising neural activity pattern as a component to learn a new task \cite{golub_learning_2018}. It takes a lot of practice to train animals to perform a task with a high level of proficiency. 

% Kaplan et al. Each has its controlling neural circuits with dynamics that control behavior rigidly

% [ ] limitations and potential fallacies of this approach 
% This discussion can be shifted to the discussion section on hcm 
% \subsection{Structure Learning as Models of Structural Perception}
%A proposal for how Structure emerges from perception

\section{Extracting structures from artificial agents}
Another direction for future work lies in looking for structures in the activities of artificial neural networks. 

% to some extent, it is proposing that any agent that learns to transfer and react to certain task in the natural world has to contains some nested hierarchical structure that is a projection of the neural world's propety on the learning agent, on plato's cave. 

% The relation between this work, LLMs, and large artificial intelligence models
In light of the recent fast development in modern AI, exemplified by Large Language Models. LLMs are gigantic scaled connectionist models trained on human language data accessible from the internet and were essentially asked to predict the association between a token of the text in relation to other tokens. Despite the simple training mechanism, they have demonstrated impressive transfer and problem-solving abilities and excelled in a set of intelligence tests that challenge highly educated humans, causing a high wave of excitement and worry about modern AI.

Part of what contributes to the worry is the uninterpretable architecture that the connectionist AI uses. This is because transformers contain millions and billions of parameters. We still have trouble understanding what makes a recurrent neural network learn to predict the next word of Shakespeare.
Uninterpretability refers to the difficulty of interpreting how computation arises from neural network models. Taking adversarial attacks, for example, visually perceptual noise in images alters a population of neural activities in small ways but alters the network's computation and change the classification from the correct to the wrong label. It is challenging to understand what makes large neural networks choose  one decision in favor of another.%, and how to interpret the neural computations carried out within 

The difficulty in understanding what contributes to the neural network's behavior makes controlling and predicting a full range of their behaviors very difficult. Because the full control and understanding of AI's behavior is out of our hands, OpenAI had trouble stopping ChatGPT from sharing bomb-making receipts; LLMs exert strange behavior when confronted with non-natural language, incongruous prompts, and spit out user private data to another stranger on the other side of the word. Finally, some of these models have been shown to exhibit biases reflecting racism and sexism that make their behavior ethically unacceptable in an open society. All of these issues have a wider impact and deeper consequences as the connectionist models are brought closer and closer to real-life applications such as autonomous driving or navigation in different weather conditions. safety, reliability, and ethics \cite{GeirhosGeneralisationNetworks,Goyal2022,lakretz-etal-2022-transformers}. The ground cause of all of the above pressing issues that is the uninterpretable nature of connectionist models. 


Existing approaches, such as using NN to interpret NN, have yielded limited success. The difficulty lies in comprehending the interaction of high-dimensional neural activities and their attributions to behavior. 
The interpretability problem bridges between neural computation and human understanding. To keep up with the fast-paced development of connectionist AI, we also need an understanding of human cognitive facilities.
Having long been an unsolved issues in connectionist AI,  researchers in connectionist AI have urged approaches that study the connection and similarities between the hierarchical structural relations that humans learn and those acquired by large-scale connectionist models in modern AI \cite{Goyal2022,Hinton2020}. % [ ] Bengio, Lekun, Marcus also have researched in this direction  

Future work can exploit our method to extract hierarchical structure in data to bridge between intepretability and connectionist AI. Three directions are worth investigation. One is to extract interpretable chunks of neural activities from connectionist systems. The second is to look for structures in the neural computation mirroring task structure. And the third is to impose rigidity and structure in the behavior of large model.

\subsection{Extracting understandable computational patterns in connectionist AI}
% use HVM and HCM as a lens of human interpretability 
Applying what we have learned about the characteristic of human understanding can shed new light into another method of interpreting large scale neural computation and activities. 

This path translates to view the proposal and findings from this thesis as what is deemed necessary to make anything comprehensible by humans: a premise of comprehension is to break observation into parts. The parts are identifiable when each of them occurs repeatedly. 
% [ ] refine that it is only in the regime of high dimensional chaotic data sequences? 

Another view to look at our tendency to chunk, to abstract, and to reuse the previously learned parts to construct the more complex, is to see this tendency as a feature of what is understandable. Endowed with our limited working memory capacity, chunking and using symbols to represent information is a means to surpass the information bottleneck imposed by our limited neural computing facilities. 

% [ ] expand a bit what specifically to do 
From this standpoint, the method of extracting chunks as repeated parts in concrete and abstract spaces can be adapted to find recurring invariant neural computation patterns amongst high-dimensional varying observations. One can, for example, start by finding neurons that have correlated activities in the artificial neural networks, look at the conjunctive activities of the neural pair in relation to other neurons or neural pairs, and gradually expand the group of neural activities under scrutiny until this is no longer possible. Thereby recurring patterns of neural population dynamics can become the basic computational unit to interpret the artificial neural activities. One can then examine the occurrence time point of such chunks of neural population activity patterns in relation to one another and look for the triggers in the input or in neural population activities that result in a cascade of patterns of neural population dynamics. 

% One marked property about equal representation is that if two representations are identified as identical, then any sort of nonlinear or linear transformation will not distort their identical relationship. One prediction is that there will be more repeated patterns in the later processing layers of neural networks than in earlier processing layers.

% [ ] what would be an evaluation measure on the effectiness of this method 
\subsection{A hierarchical structure mirroring structures in the training sequence}
An indicator of success from this approach will be finding recurring patterns in the high-dimensional neural representation corresponding to repetition patterns in the training data. Essentially, this is asking if there is a vocabulary or a dictionary of patterns represented by neural networks, then what are the vocabularies as represented in the neural activities, how many vocabularies are in the dictionary, and how does this vocabulary interact with each other during the training process, under what condition shall the neural network also represent grammatical structures as more abstract relations amongst the existing words? 

This thesis, in part, posits that our cognitive tendencies to chunk or abstract may not be just a heuristic but rather can emerge as a rational strategy for an agent discovering the structure of the environment. If this proposition is true, then it implies that other efficient learning systems, be they biological or artificial, should also acquire a representation that reflects the inherent structure of the training data. 

Therefore, one should expect connectionist models trained to predict the training data to also learn a representation that partially reflects the statistical structures within the training data. Thereby, recurring patterns and relations embedded in the training data may also be reflected in the internal neural activities of the connectionist agents. It is very often the case in natural languages that there are not just surface-level recurring patterns but also recurring patterns that are deeper and more abstract. Future work should examine neural correlations between concrete and abstract patterns in language sequences and examine their representation in a recurring activation of neural activities in models with various language proficiency. The abstract level of the connectionist model's pattern acquisition may be linked to its ability to transfer. A model that has only learned recurring patterns on a concrete level may predict concrete patterns well but fail in tasks that demand the acquisition and application of abstract patterns.  Different levels of abstract operation can emerge at various time points during training. The ability to reliably represent abstract patterns links to the model's ability to transfer its prediction abilities to novel sequences sharing the abstract but not the concrete recurring patterns in sequences. When abstract representation reliably emerges, it can be related to the 'Groking' phenomenon that large connectionist models training on abstract tasks (such as arithmetic or algorithmic binary operations) do not transfer to the test set until after an excessive amount of training on the training data \citep{power2022grokking, miller2024grokking}. Whereas the model will exert a similar level of performance proficiency in training data throughout. 
%This character of our understanding arises from the structural character of the natural world, which has recurring patterns that exist in both abstract and concrete forms. Similar categories of animals look alike, and leaves from the same plant look alike. Objects that belong to the same category tend to interact with other objects in a similar way. 

\subsection{Behaviour that distinguish biological and artificial intelligence}
This work on chunking and abstraction also highlights a marked difference in behavior between human and artificial intelligence. 

% figure: brain studying AI, rigid belief structure versus 
The rigid belief structure of humans also distinguishes them from AI. We are the animal of reason. It is not just children who are learning about the world like scientists; individual humans possess rigid and slowly updating belief systems and interpret observations via [a rigid system of interpretation], influenced by the information to which the individual has been exposed. Individuals update this belief system parsimoniously, with observation of, and interaction with, the world testing the hypothesis. And one single false example will already suffice to disprove a law under hypothesis. Although the perceived facts are subject to mistakes, people are aware of that, and collective pursuits such as science aim to develop a rigid knowledge system based on trial and error from repeated experimentation. % [ ] cite gopnik,

In contrast, connectionist AI systems learn from correlations, and hence, any prediction is considered true and false simultaneously with some probability valence. 

Also, on a behavioral level, there are strong features of human understanding that LLMs do not possess. 
While a human can't believe a fact is both true and false. Individuals seem to have been seeking laws that stand the test of time and intervention and would stand out and defend one's belief system. Humans seem to be deducing a rigid, static causal structure from data.

However, such rigidity is not processed by the large models used to this day. And this rigidity is nonetheless needed for future reliable artificial intelligence that seeks reliable patterns and tests its world beliefs in an active and parsimonious way. 

%The structure learning model can be used to build models of how humans arrive at a hierarchical perception, such as in motion data. 
\subsection{Possible Criticism}
One potential criticism of this approach is that someone might say that this particular way of interpreting behavioral and neural activities centers too much around the structure of the hierarchy itself and may be limited by anthropocentrism imposed by the hierarchical structure, leading to the danger of seeing hierarchies even when they are not present.

Statistical measures of the explainability of a hierarchically structured way of interpreting neural data need to be developed. A model will be evaluated based on its explanatory power. 

and employing this model will, unfortunately, guide a system in interpreting everything using hierarchy. 

The question is: Is hierarchy a language used by nature, or is it only a mental facilitation processed by humans to understand anything at all? 


How sequences of neural population activities encode information about object entities and relations. These recognizable patterns and relations can inform neuroscience questions about the neural underpinnings of memory representation, sequence learning, and skill acquisition. Along this line memory formation in neural computational models and the emergence of abstract representation in neural activities.



\section{Scaling up}
% learning interpretable structures from higher dimensional data 
In low dimensional discrete domains, we illustrated the power of recursively combining the previously learned representation to construct more complex ones, allowing learning interpretable representation. Future work can adapt and extend this representation learning principles to higher dimensional data domains. 
% this section is going to the discussion of HCM 
\subsection{Tokenization}
The chunking principle can be referred to as enhancing the learning of connectionist models. In these machine learning models, a widespread practice during the preprocessing of natural language data before training is to tokenize the dataset. Tokenization methods, including byte-pair encoding, or xxx, are essential for data preprocessing to train transformers. The mechanism is very similar to chunking: frequently-occurring, words or word parts, are grouped as units of tokens. Each token spans several sequential units. The processed sequential tokens are then assigned specific integers as the input sequence to train transformers. Empiricially, works have shown that the tokenization process is criticial to efficiently train large language models. As we demonstrate the effectiveness of chunking in our work for compression, abstraction and transfer, it also give hints to tokenizer's effectiveness in preprocessing the training data. 

If chunking data can help with neural network training, future work can also look at chunking data at different levels of processing, in addition to the role of abstraction in helping with training. For example, as tokenization is usually only done on the training data once and never occurs again, tokenization on the intermediate level of information processing in the neural network may help the neural network's learning to progress faster. Additionally, it can be interesting to test the effectiveness of tokenization not only on a concrete level but also on an abstract level to examine if layers of preprocessing in both concrete and abstract tokenization levels can advance neural network training even further. 

\subsection{Acquiring modularized representation from high dimensional data}
The second direction in scaling up aims to extract interpretable and modularized representation in high-dimensional data.

% where to apply it 
In the visual-temporal domain, the chunking principle can be used to learn motion structure and video component segmentation. Particularly, motion elements that share a similar spatial and temporal profile would be grouped together in a memory resource rational way. In the sound modality, chunking can be applied for speech segmentation and music perception. Other applications of the chunking model can be learning proprioception data or inferring value functions from observation states in reinforcement learning. 

% why is it worth thinking about it
Past work in computer vision has used modularized representations of natural images. Starting with learning independent components of natural images. A line of work in CV aims to look for a grammar that describes visual images (Zhu et al. )(examples of such primitives can be a Gabor bank or a set of steerable filters). And object identification from natural images becomes identifying patterns that are consistent with an image's grammar. A modularized representation of high-dimensional data, such as natural videos, contains many benefits, including a structured explanation of the composition of object categories and improvements in data efficiency and transfer. 
% how to apply it 
It is worthwhile to give modularized image representation another shot, integrating chunking and contiguity principles with the current state-of-the-art machine learning methods. 

A modern version of this approach can adapt chunking with existing neural network methods that are capable of processing high dimensional fidelity data. For example, the chunking principle can be applied to representations lying in an intermediate layer that has been disentangled in some artificial neural space, bridging the structure between high dimensional input to neural network to low dimensional symbolic and structural representations. This may help the model to arrive at an object-based representation and enable learning of the relations that are defined on top of the objects.

Apart from applying chunking to representations that are already low dimensional by having been processed by a trained neural network, the chunking principle can also be adapted to process high dimensional data. Towards this direction, the grouping principle may need to be flexibly adapted to account for the high variability in natural images. For example, chunking based on frequent transitions can be applied on the level of spatiotemporal attention masks in transformers \cite{Vaswani2017AttentionNeed}. Additionally, introducing grouping by visual similarity may also be necessary to empower the model that learns part-whole hierarchy. This direction aligns with work on image segmentation and object representation using a combination of neural networks and spectral graph theory approaches. My previous work has demonstrated the relation between weighted graph representation of images and human vision: the computational steps of a weight graph cutting algorithm correlate with the visual recognition difficulty of amorphous image parts.

This model provides a more interpretable and generalizable representation of the video as it explicitly decides whether or not to chunk parts of the video together for prediction, leading to modularized explanations and isolations of video sequences. Models adapted in such a way may be capable of disentangling various motifs, such as isolating movement tricks that are oftentimes combined with each other to perform a skateboard trick. 

The tendency of grouping by proximity and similarity may contribute to the shape bias in human vision, as shown to distinguish from the texture bias exerted by machine vision, as similar textures may be combined together for a more resource-saving description of a natural image \cite{Geirhos2018GeneralisationNetworks}. Toward this direction, integrating the grouping by proximity or similarity principle with the state-of-the-art image classification networks could produce more human-like visual classification more robust to noise perturbations \cite{Goodfellow2014ExplainingExamples}.

% delete
% In the era of deep learning, both natural language processing and image processing became increasingly dominated by neural networks, with one of their primary tasks being the extraction and prediction of chunks \citep{Zhai2017NeuralMF, Si2020, Ortmann2021ChunkingHG}. Commonly, these so-called sequence chunks are used as units of segmentation for other downstream tasks such as text translation. However, in these approaches, the architecture needs to be pre-specified before training as compared to HCM, where no such specification is required. HCM can therefore be seen as an interpretable and transparent alternative to neural networks for some of these tasks.

%moreover, for neural networks, knowing and retrieving the type of chunks always comes with additional work that has been acquired during the training process and what can these representation say about the performance in an alternative environment has always been a challenge. The transparent, interpretable, and compositional aspect of HCM helps to answer such questions. 


%For example, HCM can work as a backend of the output of a neural network or a transformer to learn chunks within a latent space. Another possibility is to learn chunks of output labels such as animal movements to discover patterns underlying these labeled parts \citep{insafutdinov2016deepercut}. The learned chunks can become structural hypotheses for causal discovery \cite{Heinze-Deml2018CausalLearning, scholkopf2021toward}, subject to experimental interventions or active learning.

% Grouping images by parts and wholes have also been suggested in computer vision approaches for image segmentation \citep{Shi2000}. We are actively working on integrating HCM with features that make the representation structure more adaptive, such as adding translation or rotational symmetries or integrating with computer vision algorithms such as coherent point drift, and in the future to employ the merits of these algorithms. 



% more flexible measures of chunking in natural images should be adapted. 
% some neural network behavior resembles more to humans, some don't, it is unclear how and why they do and don't 

% \subsection{Bringing neural network closer to humans by reusing previously learned concepts (as much as possible)}
% \section{Towards a probabilistic representation}
% \label{sec:conclusion:sec1}
% This work does not consider the scope of probability. 

% \section{Adding a valence of reward and punishment}
% \label{sec:conclusion:sec2}

% \section{Other improvements}
% \label{sec:conclusion:sec1}
% This work does not consider the scope of probability. 
% Adding a probabilistic representation and integrating it with Bayesian inference. 

% Adding a valence of reward and punishment

\section{The limitation of symbolic representations}
% I will use the final section of the discussion section to talk about the limitations and potential fallacies that may be introduced by hierarchical representations. 
%This thesis studies how compositional primitives arise and how primitives can be reused to construct more complex sequences. However, we also need to be aware of the limitations of using compositional and symbolic representations to see the world or solve a problem.

% There are multiple ways to learn primitives, and the biological ways of learning primitives may not be the optimal way of discovering primitives in data. HUman cultures also evolved from different sets of primitives. 
For one, the set of primitives that are learned in a dictionary, or a composition of primitives in the dictionary, is a particular way of breaking down observation into parts. With our algorithm, we propose a way of learning primitives, but it is impossible to verify the optimality of which set of primitives to learn that gives us a ground truth representation of the world. Because when it comes to natural sequences, there is no underlying ground truth. However, we usually rely on a conventional assessment of object identification or relational identification as offered by the convention of the current civilization and the current popular language or culture we are embedded in to study the topic. This would imply that alternative cultures, as separately trained learning systems, would identify concepts differently than other cultures. Consider words that exist in some languages but do not exist in alternative languages, which suggests an independent learning of primitives. 


Another dimension of symbolic representation is the loss of information. 
However, by representing observation as symbols stored in some cognitive dictionary, we can quickly make sense of the world and use less mental capacity. However, a purely symbolic representation of the world would, by definition, contain a loss of the subtle nuance of perception itself. As symbols are a way of extracting features from the observation, there are alternative ways of extracting features. Our tendency to perceive things as what we want to see (or what we already know) will hinder us from perceiving things as what they are. 

Another implication of reasoning and deduction in symbolic form is that it limits understanding to things that cannot be expressed in symbolic form. Many things, such as beauty, aesthetics, and music, cannot be expressed in symbolic form, so they are, unfortunately, excluded from a discussion operating on the basis of symbols. 


Symbolic representations are unfortunately unmealable, and the consequences are not always positive. 

% \section{System Section 3}
% \label{sec:system:sec3}


% \section{Conclusion}
% \label{sec:system:conclusion}


%\section{What this thesis is not}
%\subsection{Models are non-probabilistic}
% hence don't fit it to humans individually 
%Because the integration of probability into a noisy algorithm will only hinder a good understanding of it. Probability is an add-on, but it creates unnecessary burden as the first step to tackle a question. Hence towards answering the above two questions, we do not develop algorithm that integrate probability. While probabilistic algorithms are useful to characterize a distribution of human behavior. We reserve this aspect of work to the future and focus on simplifying the understanding for now.  

% Bayesian inference explains how knowledge guides inference from incomplete data. But in all cases, questions remain as to how could structured symbolic knowledge be acquired through the process of statistical learning from sequential data (\cite{tenenbaum_how_2011})


%\subsection{We don't consider rewards, yet}
%Although I think it makes a sense that structures are tied to reward, and there are some unnecessary structuresstructures to learn unless they can be associated with reward and punishment. This thesis takes the reductionist approach and first considers the benefit of teaching structures purely in the statistical sense from perceptual sequences. 
%We reserve the study of reward to other approaches for future work. 

%\subsection{It is not hierarchical clustering}
%In some literature, chunking is also referred to as grouping. 
% We don't try to work with super high dimensional data; the entire thing is more meant for a conceptual demonstration 




==> content/ex-chapter-introduction.tex <==
% !TEX root = ../thesis-example.tex
%
\chapter{Introduction --- the commonalities between associationism, Gestalt laws, universal grammar, chunking, and their algorithmic advantages}
\label{sec:intro}

\cleanchapterquote{The propose of science is to find meaningful simplicity in the midst of disorderly complexity.}{Herbert Simon}{}

%From a lot of sensory input, people make sense of the world. [Temporal data, non-iid, timeseries, sequential]
%How people do this has been a core question of philosophers and psychologists alike. 
%Some philosophers argued that people are rather tabula rasa. They start out like a blank sheet and gradually makes sense of the world. But how would they do this? Philosophers argued that they do this via rules of association (see Hume) and abstraction (all the way to Aristoteles).  [interesting because your model is kind of tabula rasa (atomic units) and learns via association (Hume) and abstraction (Aristoteles)]
%Psychologists have long been fascinated by how people make sense of the blooming and buzzing confusion. 

% [ ] only capitalize the first letter
\section{A long-standing question}
\label{sec:intro:motivation}
%From a lot of sensory input, people make sense of the world. [Temporal data, non-iid, timeseries, sequential]
%We effortlessly perceive entities from an immense volume of an ever-changing sensory stream. Imagine sitting on a stone in the mountains during a hike: successive sensations arise from an influx of perception. You witness the expansive view of mountains, hear the delicate chirping of birds, sense your pounding heartbeat, and feel the tickling itch of a mosquito bite. Despite this overwhelming flood of sensation, cognition seems to skillfully sift through the sensory stream, catching and identifying meaningfully structured entities that momentarily emerge and fade.
% This remarkable capability to navigate and interact with our complex environment with ease can be partially attributed to our ability to organizing sensory information into manageable units and distilling meaningfully structured patterns .

We effortlessly perceive entities from an immense volume of an ever-changing sensory stream. Consider the process of walking through a bustling city: successive sensations arise from a continuous influx of perception. You notice the swift changes in traffic lights, hear the diverse sounds of car horns, feel the differences of the surfaces you are walking on, and smell the fleeting aroma of a nearby food stand. Amidst this overwhelming flood of sensation, cognition skillfully sifts through the sensory stream, identifying concrete entities such as "traffic signals," "road conditions", and "food stand". This remarkable capability to navigate and interact with a complex environment with ease relies heavily on our ability to distill meaningful patterns from sensory streams. 

How people make sense of the continuous stream of sensory inputs has puzzled philosophers and scientists for centuries. Aristotle defined those perceptual entities as categories abstracting away from the first-hand perceptual experience, entities for inducting and deduction of new knowledge beyond our limited perceptual experience \cite{aristotle1938,AristotleAnalytics,AristotleCategories,AristotleInterpretation,AristotlePosteriorAnalytics}. 

% hume, locke: understanding is constructed from experience 
The British empiricists notoriously underlined the importance of experience for the acquisition of knowledge \cite{hobbes1651, locke1690,hartley1749,mill1829,mill1843}:
John Locke initiated that newborns process a blank (\textit{tabula rasa}) state of mind, in which perceptual entities and categories emerge from experience \cite{locke1690}. Hume delineated this process as perception come first to the mind as vivid ‘impressions’ and later distill into more abstract and less lively ‘ideas’. Abstracting and associating ideas then becomes the building block of more complex mental structures \cite{hume1777}.
% % hume, locke: understanding is constructed from experience 
% At a later stage of philosophical development, the British empiricists were also interested in the acquisition of categories, notoriously underlining the importance of experience for the acquisition of categories. 
% John Locke initiated the tabula rasa theory: newborns process a blank (\textit{tabula rasa}) state of mind. Perceptual entities or categories emerge solely from experience and learning associations while experiencing the world \cite{locke1690}. Hume later delineated a process of abstraction by describing perception as vivid ‘impressions’ that come first to the mind and later develop into much more abstract and less lively ‘ideas’. The empiricists proposed two laws of association that connect ideas through experience: two events are associated if they occur in spatiotemporal proximity (\textbf{Law of Contiguity}). The strength of association is determined by the number of repetitions (\textbf{Law of Frequency}) \cite{hobbes1651, locke1690,hartley1749,mill1829,mill1843}. Associating ideas then becomes the building block of many mental facilities. By learning associations between impressions observing one event succeeding another, relations such as causation, can be proposed from experience being further tested by intervention \cite{hume1777}. By abstraction and association, categories and structured relations between ideas develop through accumulating the experience sequentially observing and interacting with the world.

% [ ] link back to it during the discussion of the model 

% [ ] figure: the emergence of structured ideas from human perception 


\section{We learn associations and structures from multiple psychological modalities}

% [x] Law of contiguity 
% [x] skinner
% [x] throwndike 

When mental processes become a subject of study for psychology, Locke's tabula rasa description of the newborn is transformed into the question of how babies 'make sense of the world'. Described famously by William James as a "great blooming, buzzing confusion.", newborns face the demanding challenge of understanding the world from the noisy and transient sensory experience. After a while, they tend to gradually figure out a way to identify a coherent understanding of objects and execute a sequence of actions to interact with those objects proficiently. 


%ractice, forgetting, temporary extinction, emotional reinforcement, irradiation, response to patterns, and alleged insight, 
%He concludes that these may all be understood as instances of the principle of association by contiguity in time.

The empiricists' postulation of structures arising from experience was taken up by the behaviorists in search of principles that generalizes the nature of learning. They remarked a primary feature of learning is by learning association between stimulus pairs. 

Pavlov observed that dogs' capability to form a new association between pairs of stimuli through repetition and reward. While dogs naturally salivate when presented with food, an unconditioned stimulus, repeatedly pairing the sound of a bell, a neutral stimulus, with the food, they eventually associate the sound of the bell with the arrival of food, salivating at the sound of the bell alone, even when the food is absent \cite{pavlov1927}.
In such a way, animals acquire new behaviors and responses through repeated pairing between stimuli. 

The behaviorists propose that the effect of practice, forgetting, and response to patterns can be understood as instances of the Law of Contiguity \cite{guthrie1930}: after events occur in spatiotemporal proximity, the reoccurrence of only one event evokes the memory of the others. Through experience, successive sequences of actions tend to be associated with each other. 

This law was first demonstrated in animals. 

Thorndike's summarized  \cite{thorndike1913} three factors that influence associating stimuli with responses: (1) the law of effect states that responses to a situation followed by a rewarding consequence will be strengthened and become habitual; (2) the law of readiness states that a sequence of actions can be chained together and (3) the law of exercise states that the connections between actions become strengthened with practice. Thorndike suggested that such sequences of connected responses transfer to the animal's response in a new environment when similar situations occur. Later, Skinner refined the concept by adding the consequences of behavior as another factor. I.e., the animal's behavior is weakened or strengthened by the immediate consequences of that behavior. When the immediate consequences are positive, such as obtaining food, the behavior is strengthened (positive reinforcement) \cite{skinner1953}. When a similar situation occurs again in another instance, the situation is sufficient to trigger the idea of that movement. Through repeated experiences and reinforcement, animals form behavioral patterns and seamlessly execute a sequence of complex responses based on past experiences. Thorndike foresaw the theory of contiguity to cover almost all areas of learning, \cite{thorndike1927,thorndike1928}, language comprehension \cite{thorndike1921} and mathematics \cite{thorndike1922}.% To today, the Law of Contiguity is still considered a keystone of most theories of learning, memory, and knowledge.


% reviewing the cognitive science literature
\subsection{Learning structures in other sensory domains}
%[ ] Structure 

% [ ] The idea of "just continguity" has been severally criticized by linguists, see Chomsky
\subsection{Structures in language}
% [ ] merge is the minimal universal grammar 
% structures underlie language, 
Language is another modality in which structure prevails beyond vision and behavioral responses to stimuli. 
A set of paradoxical characteristics underlies human language. On the one hand, language is infinite. We are capable of uttering novel sets of clauses and judging the grammatical and validity of a vast number of previously unheard sentences. %Given a previously unseen sentence, we effortlessly say whether they are grammatical or agrammatical. 
On the other hand, relative to the infinite amount of varieties that language itself affords, linguistic input available to children is limited. Despite this \textit{Poverty of the Stimulus}, children can utter new sentences with valid syntactical structures. This ability cannot be achieved by simply memorizing all previously heard sentences \cite{Chomsky1965, Chomsky1980}.
In contrast to the infinite combination of languages is the finite amount of memory we possess. 
How would such an infinite amount of sentences generated with finite memory sources?

Despite the vast differences in languages across the world and their diverse grammatical forms, one remarkable characteristic of language is the pattern in both concrete and abstract forms. One cue of how language can be learned by the mind is to learn structure on multiple hierarchical levels \cite{fitch_artificial_2012}. On a lexical level, most languages are made of words composed of a finite set of basic symbolic elements, such as the alphabet in English. Letters in the alphabet combine together into word parts, such as 'tion', 'ish', 'ly'. The next level of organization is words, which populate the entries of lexicons. 
% phrase level 
On a phrase level, the structure continues, words combine together into phrases, such as 'in doing so', or 'once upon a time'. Beyond phrases, on a sentence level, grammatical rules specify combinations of patterns of word categories into valid sentences. 
Such as the third person singular in the simple present tense always ends in –s, or a sentence always contain the components 'subject' + 'verb' + 'object'. At each level of organization, whether it is on the level of alphabets, words, phrases, or sentences, the existing elements in the organization then combine together into more complex composites. The product of the composition and the variety of outcomes increase with the level of hierarchy. 


% Learning associations and seeing structures are also manifested in the language modality. The thesis connects merging and hierarchical structure with gestalt psychology and learning associations. 


\subsection{Regularities help action execution}
% [ ] talk about the benefit of structure in one paragraph 
Another domain of our behavior in which structure prevails is in action. Our daily actions contain hierarchical structures that span across short and long time scales. An action as simple as making a tea would naturally involve steps including getting a tea bag, boiling hot water, pouring the water into the tea, waiting for a couple of minutes, taking the tea bags out, and finally drinking the tea. Substeps are embedded in each step, such as getting a teabag, which involves finding a tea box, opening the tea box, taking one tea bag out, and closing the tea box. This complex series of movements comes to us so easily and effortlessly that we execute it without a second thought. 
Theories formulate planning as an agent selecting a set of executable actions that allows it to reach from a source state to a goal state \cite{laird1984towards}. In planning, when we would like to reach a goal state, such as drinking tea, then the goal state can be composed by chaining together sequences of sub-goals. The mastery of execution sequences that allow the arrival of sub-goals enables a combination of existing skills to accomplish an otherwise much more complex goal \cite{Tomov2020DiscoveryPlanning, Wiener2003,Balaguer2016}. 


\subsection{The structured organization of memory}
% [x] memory is organized into chunks
% [ ] Miller, michael frank, mirroring earlier literature discussions
% [x] dehaene

% % humans are sensitive to association between nearby occurrence of items 
% In memory, statistical learning (the learning of the transitions between items) is a powerful way to detect and exploit regularities in sequences. 

% memory of sequences is organized into chunks, and hierarchical recursive abstract structures  The emergence of sequence parts into cognitive units. 
Mirroring the structures in our action sequences, language usage, and perception, is the structured organization of our memory. 
When remembering sequences, we tend to break the sequence into several chunks. A continuous stream of perceptual input is segregated into concrete parts, memorized, and recalled as separate entities. About half a century ago, Miller discovered an interesting relationship between chunks and short-term memory. While it is generally known that humans have a limited short-term memory span, Miller discovered that the unit of short-term memory storage capacity is in chunks. Broadly speaking, a chunk is a grouping of several sequential elements as one entity that can be recalled as a unit \cite{Mathy2012WhatsMemory}. On average, people can hold from 4 to 7 chunks \cite{Miller1956TheInformation}. This implies that longer chunks help us to remember longer sequences. Imagine having to remember the sequence ``052917080461''. Taken on its own, this sequence might be difficult to remember. However, knowing that it contains both John F. Kennedy's and Barack Obama's date of birth will likely simplify remembering the sequence. Even small babies learn to segment language. Chunking allows subjects to store a longer sequence within a limited resource of short-term memory and functions as a basic unit of cognitive processing. 

Studies have suggested that humans memorize sequences using a nested hierarchy of smaller chunks embedded into bigger chunks \cite{Planton2021}. Past research has observed this grouping of several stimuli entity as one coherent unit in sequence learning, grammar learning, visual, and working memory tasks \cite{Miller1956TheInformation, Rosenbaum1983HierarchicalSequences,Lashley1951TheBehavior,Graybiel1998TheRepertoires,Halford1998ProcessingPsychology,Gobet2001ChunkingLearning,Dempster1981MemoryDifferences,Schyns1998TheConcepts,Wickelgren1979ChunkingSystem, Egan1979ChunkingDrawings, Ellis1996SequencingOrder, Bor2003EncodingDemand, Jin2014BasalSequences, Grainger2011AProcessing,Penhune2012ParallelLearning, Orban2008BayesianObservers, Dehaene2015TheTrees, Brady2009CompressionRepresentations, Verwey1996BufferKeypressing, Koch2000PatternsTasks, Terrace1987ChunkingTask,Gobet2001ChunkingLearning,Gobet2004ChunksTwo}.

%suggesting chunking to be a cost-saving strategy that enhances effectiveness of symbolic sequence learning \cite{solopchuk2016}. 

% By simulating interactions between ideas, we are able to foresee consequences and make decisions accordingly. By applying the learned relations between ideas, we reason inductively and express ideas through language. By recombining existing ideas in uncommon ways, we create imaginations out of reality. 

%The reorganization of those perceptual stimuli representations enables the categorization of the perception into a rather natural hierarchy.    

% while reading, we make use of the regularities 
As it is the case that we observe the composition of the symbolic form of language, it is also the case for how we understand languages. When we read a sentence, nobody parses a sentence letter by letter. Rather, parsing of the sentences tends to happen on a word level or even on a phrase level, as observed also by linguists studying the eye movements as people read. During reading, we shift our gaze along each line of text so that successive chunks of words are processed in high acuity \cite{paterson2020}. Upon processing a complex symbolic sequence,  we use the regularities and parse sentences on a chunk-by-chunk level. When there is a sentence composition that does not fit our expectation of a grammatical structure, it triggers an inherent discomfort to be acutely aware of reading something violating the regularities we expect. 

% \cite{planton_theory_2021} conducted a series of experiments to evaluate the mental compression of bindary sequences in an odd-ball detection task. They varied sequence length and sequence sensory modalities, and showed that sequence encoding performance (as measured by sequence deviation detection) can be explained by the length of the shortest possible description of the sequence in their proposed LoT measure. Their results supports the idea that upon hearing or seeing a binary sequence that spans beyond working memory capacity, a model that represents binary sequences using 'same' or 'change' and their recursive embeddings can account for a large variability of subjects' behavior. 


\section{The computational benefit of structure and symbolic representations}
Psychologists and philosophers alike have noticed that humans naturally have a set of interesting tendencies to perceive discrete structures from perception, which is fundamental to our thought processes. This raises the question of why a concrete structure should support cognition and observation representation. Interestingly, this question is studied extensively in the fields of computer science and artificial intelligence. 

\subsection{Classical AI started with symbols}
%The initiation of artificial intelligence as a field started with operation of symbols.
% herbert simon noticed this behavior and tried to understand the computaitonal principles behind it. 
A lot of science is about looking for invariances in physical phenomena; Herbert Simon also proposed to look for ‘invariants’ in human behavior. He posited that a system will only be capable of intelligent behavior if it is a physical symbol system, operating on symbol structures via input, output, storage, modification, and manipulation via action, namely, the Physical Symbol System Hypothesis \cite{Simon1990, Newellsimon1976}. He proposed to look for invariants in human behavior, one should show the process by computer programs are the same as what people used to perform certain task. 

The limitation of our ability to process symbolic information translates to processing half a dozen chunks within our short-term memory. He proposes to reduce the computational requirement upon solving a task with our bounded computational resources, one should store knowledge in long-term memory and retrieve knowledge upon recognition. When there are problems with solutions not immediately provided by recognition, heuristic search is yet another proposal of how humans arrive at an expectation of the solution at hand, given a combination of existing knowledge. 

% the early AI stuff are all symbolic, like mathematical deduction, equation solving, even natural language, and image processing tends to use a set of symbols to represent data, and then studying the manipulation of these symbols

\subsection{Symbolic systems factorize distributions}
% symbolic representation introduce factorized representation in computer science? 
When an algorithm needs to process high dimensional distribution such as $P(x1, x2, …, x_n)$, it implies computing a complex global function with many variables. One strategy for reducing the computational time and cost is to factorize the high-dimensional distribution into independent groups of random variables. $P(x1,x2)P(x3,x4)P(…, x_n)$ —— dividing a big complex problem into several independent smaller problems, a global function into several local functions. The structure of the distribution can then be described by a factor graph. An estimation, such as computing the marginal distribution of a subset of the variables, can be computed by a message-passing algorithm. Message passing as an operation on the factor graph also translates to Markov random fields, bayesian belief networks, message passing also translates easily to belief propagation Algorithm, Viterbi algorithm, and Kalman filter \cite{Kschischang2001FactorAlgorithm, Aji2000TheLaw}, and learning a structural causal model that generates data. 

The computer science literature suggests an efficient way of estimating a probability distribution is by factorizing it; this trick especially works with distributed computing systems. 
When estimating a high-dimensional probability distribution, the best way to efficiently calculate it is by factorizing it. A computing system just needs to compute the independent contributing factors to the distribution. 

% symbols are related to the parts in causal graphical models, which is another branch that tries to extract interpretable representation as good models for data. 
%The literature of probabilistic graphical models and causal inference provided a proposal for the inference of Probabilistic entities based on observation. Usually, the entities in the world are described as a set of random variables. The dependencies of some variables on others are described as the conditional probability of a variable conditioned on a set of other variables. 
% yet this branch is also still researching the origin of structures, i.e., where do causal graphical structure come from

\subsection{Symbolic Models are data efficient}
% [ ] SC Zhu's work, and other works on symbolic learning , [ ] holyoak's work, [ ] automatic program prover, [ ] copycat 
Because symbols are a natural way of factorizing data, symbolic models are very good at learning from limited data. For example, the Bayesian program learning framework \cite{Lake2015Human-levelInduction,ellis_dreamcoder_2020} uses a composition of primitive programs to represent observations, building rich concepts compositionally from simple primitives.
These approaches are very data efficient; symbolic models can transfer by recomposing the existing symbolic program very few training examples and resemble human behavior in some cases. 


\subsection{Symbolic systems can be easily transferred and generalized}
Symbolic approaches to modeling human behavior combine the distribution factorization idea with compositionality. This is because symbols are natural ways of factorizing data, and with concrete symbols to describe data, composing symbols becomes an explicit process. And the benefit of compositionality lies in solving tasks that are non-existent in the training process that are reachable by combining existing symbolic factorizations, when these symbolic factorizations can be readily reused.

This is the reason that program induction models exert the abstraction ability of applying the same program to different inputs, which enables generalizing and transfer. For example, dream coders have found ways to synthesize programs that edit text, such as taking the suffix of phrases (Alan Turing -> A.T. Grace Hopper —> G. H.). This is because the programs that build up the primitives can be applied to a variety of inputs, thereby enabling flexible exchange of the data item that applies specifically to programs. Hence, transferring the same program to different inputs is beneficial, and the learning is not constrained to one specific input. Symbolic models also capture the ability to generalize concepts using just one example and use concepts in very rich ways. 


The symbolic representation also is interpretable and enables the learned symbolic concepts to combine in previously unseen ways. 

% Humans have the astonishing capacity to quickly adapt to vary- ing environmental demands and reach complex goals in the absence of extrinsic rewards. Part of what underlies this ca- pacity is the ability to flexibly reuse and recombine previous experiences, and to plan future courses of action in a psycho- logical space that is shaped by these experiences. 

%There are a set of approaches on cognitive structures. 


%Compositionality offers a framework to compose the infinite out of finite means. But there comes limitations with this approach. For one, the program induction framework relies heavily on the assumption of having a library of primitives, and usually, such library of primitives are designed by domain experts. 

%Another problem is that the method to combine primitive functions are usually executed by a search process. This search process is usually very computationally demanding. 


% grammar induction 

%Symbolic models that reuses, and composes include the program induction, grammar induction, and some models in language learning. 
% there are some models that suggests how new structure can be composed from simple primitives 

%Bayesian program learning framework has been mostly applied to domain-specific programs, such as a library of the basic movements needed to compose the possible handwritten characters, symbol composition in vector algebra, or simple LOGO graphics. The program induction framework does not suggest where the initial primitives or symbols come from. 

% But there are no models that suggest how primitives and a composition of primiitves can directly arise from data/ 

% symbols, if they are important, shall also emerge as entities in connectionist architectures 

% Marr


\section{The current proposal}
\label{sec:intro:problemsetup}
% \section{Studying sequences}
% motivate sequences 

The current thesis puts the problem of the emergence of structured representation from data in a sequence learning setting. A continuing stream of perceptual inputs is segregated into concrete parts, memorized, and recalled as separate entities. Sequence processing, perceiving, memorizing, and retrieving temporally ordered series elements is omnipresent in all human activities, from memorizing and recalling events and generating action to the usage of language and music. Patterns emerge as a unit with repeated practice. We have a particular ability to generate and identify patterns and segregate coherent units from perceptual streams. 


% the approach from this thesis:
From philosophy, psychology, and cognitive science, we learned that perceiving structured patterns from data is the most pronounced mental construct that underlies all domains of perception and cognition. From computer scientists and cognitive modeling, we learned that structured representation brings computational benefits such as transferability, compositionality, distribution factorization, and data efficiency.   

% the unsolved problem before the thesis 
However, in psychology, we do not know why learning associations and structures can be beneficial for cognition. In computer science, we do not know how the structured representation arise from data. And what could be a connection between learning associations, chunking, gestalt rules, compositionality, distributional factorization, and generalization? What could be a rationality justifying our inherent tendencies to learn associations and break sequences into structured discrete components?  

% Perspective of this PhD work from the point of view of Marr


The thesis put forth a proposal to answer the above two questions. It posits a hypothesis that structures in perception arise from computational principles of rationality. It suggests an underlying nested hierarchical structure inherent in perceptual sequences. So much so, that a rational learning agent should acquire chunks and abstractions from perceptual sequence as cognitive entities. To do so, the thesis puts forth a proposal on how learning association and information abstractions bridges complex sensory sequences to discrete and structured representations, bringing forth computational efficiency and transferability. 

Specifically, this question is addressed in two parts. The first part studies the emergence of chunks in cognition. The second part studies the emergence of abstraction. For both parts, the questions are approached in conjunction with conducting cognitive experiments while constructing a model to demonstrate the employability of the computational principles. Specifically, the chapters are divided to address the four submitted projects that have resulted from this PhD work: 

\textbf{The emergence of chunks} 

\textbf{Chapter \ref{sec:srt}} introduces the project in which we study chunk learning in a serial reaction time task. In this task, chunks are inferred from the speed up in reaction time. We manipulated the underlying statistical structure of the sequences and instruction demands. We discovered that humans adapt their behavior to the statistics of the sequence, and learn longer chunks when there are longer underlying chunks in the sequence. Meanwhile, instruction of focusing on speed and accuracy also modulates human chunking behavior. We came up with a simple model that learns chunks and optimizing a utility function that includes both speed and accuracy to understand human behavior.  
\begin{itemize}
    \item "Chunking as a rational solution to the speed-accuracy trade-off in a serial reaction time task" (Wu, Éltető, Dasgupta, \& Schulz) was published in \textit{Scientific Reports} \citep[][; doi:10.1038/s41598-023-31500-3]{wu_chunking_2023}.
\end{itemize}

Taking inspiration from what we learned in human behavior, the second project discussed in \textbf{Chapter \ref{sec:hcm}} takes chunking further under a normative lens. It studies sequences with an underlying nested hierarchical structure and proposes a model that uses chunk learning by association to uncover the underlying nested hierarchical structure in sequences. The principles resulted in a model that recursively reuses the previously learned representations to construct new ones. The work also generalizes chunking from a one-dimensional sequential domain to a visual and visual temporal domain and illustrates its potential to be applied as a data-driven structural discovery algorithm. This work resulted in the following publication: 
\begin{itemize}
\item "Learning Structure from the Ground up—Hierarchical Representation Learning by Chunking" (Wu, Elteto, Dasgupta, \& Schulz) was published in \textit{Advances in Neural Information Processing Systems} \citep{wu_learning_2022}.
\end{itemize}

The second half of the PhD work studies abstraction in sequences. 

It starts with a sequence memory and recall experiment \textbf{Chapter \ref{sec:motif}}. This defines two types of motifs and studies the influence of motifs in learning to memorize and recall long sequences, in addition to transferring motif knowledge to novel sequences. The sequence recall experiment suggests that people seem to exploit sequential patterns and redundancies not only on a concrete, but also on an abstract, level.
\begin{itemize}
    \item "Motif Learning Facilitates Sequence Memorization and Generalization" (Wu, Thalmann, \& Schulz) is available as a preprint on \textit{PsyArXiv} \\ \citep[][;doi:10.31234/osf.io/2a49z]{wu_thalmann_schulz_2023},  and, at time of submission, is under review at \textit{Communications Psychology}
\end{itemize}

The experimental work inspired more modeling of human abstraction learning and inspired its connection with learning by association and chunking. The last project discussed in \textbf{Chapter \ref{sec:hvm}} studies both abstraction and chunking under a normative perspective. A learning agent should propose to discover categories from its observations because naturalistic sequences contain distinct objects of the same category type. Such properties enable the learning agent to learn patterns from sequential data layer by layer on concrete and multiple abstraction levels. The work also relates abstraction with generalization and distinguishes large language models' learning and transfer behavior with cognitive models. 

\begin{itemize}
    \item "Building, Reusing, and Generalizing Abstract Representations from Concrete Sequences" (Wu, Thalmann, \& Schulz) is a submitted manuscript \citep{wu_thalmann_schulz_2024} and, at time of submission, is under review at \textit{Advances in Neural Information Processing Systems}
\end{itemize}

Some works are related to the thesis topic developed during the PhD, but are not discussed in the thesis. This includes our approaches in two directions: 


One is to test the applicability of chunking principles in biologically realistic simulated neural circuits. I worked with Atilla Schreiber, Chenxi Wu, Giacomo Indiveri, and Eric Schulz to demonstrate a group of spiking neurons with biologically plausible principles of synaptic plasticity and homeostasis can learn structured patterns from sequences in mixed-signal neuromorphic hardware. The project suggests that biological neural circuits and computation structures are capable of learning chunks in computationally and power-efficient ways. 

\begin{itemize}
    \item "Biologically-plausible hierarchical chunking on mixed-signal neuromorphic hardware" (Schreiber, Wu, Wu, Indiveri, \& Schulz) was presented at the \textit{Machine Learning with New Compute Paradigms} conference \citep{schreiber2023biologicallyplausible}.
\end{itemize}

The other work takes into account grouping by similarity and tests structure learning from a hierarchical-dimensional visual modality. In a novel psychophysics paradigm, I worked with Mehmet Yurueten to study subjects' recognition behavior upon seeing images tiled by amorphous sub-parts.  We relate the recognition difficulty of image parts with the computational resources of the normalized min-cut algorithm needed to solve an optimization problem of grouping by similarity.

\begin{itemize}
    \item "Normalized Cuts Characterize Visual Recognition Difficulty of Amorphous Image Sub-parts" (Wu, Yoerueten, Wichmann, \& Schulz) was presented at the \textit{Computational and Systems Neuroscience (COSYNE)} conference \citep{wu_yoerueten_2024}.
\end{itemize}


Together, this thesis proposes how structured representation in chunks and abstract rules arises from learning from discrete sequences. It suggests an underlying nested hierarchical structure inherent in perceptual sequences to be discovered as a rational learning agent. The means to do so is via learning association to construct chunks and propose abstractions as cognitive entities, bringing forth computational efficiency and transferability. 





==> content/ex-chapter-model.tex <==
\newcommand{\B}[1]{\mathit{B}_{#1}} % notation for the belief set
\newcommand{\zero}{\emptyset}
\newcommand{\Pro}[1]{P_{\A{#1}}}
\newcommand{\mc}[1]{\mathcal{#1}}

\chapter{Chunking, from simple to complex $\times$ concrete to abstract}
\label{sec:models}

% \cleanchapterquote{}{}{}
\section{Characteristics of sequence learning}

We gather knowledge from the literature to construct a structured learning model with minimal but reasonable assumptions about cognitive capabilities and examine, through experiments, the model's resemblance to human and other learning agents' behavior. 

%Human sequence learning behavior has been characterized by learning associations and learning chunks. 
% [x] associative learning models
%The TP between two syllables, X and Y, is the probability that given one of the syllables, the other will also occur. 

% [ ] make better
The first feature of human sequence learning suggests that we can adapt to simple sequence statistics, including the occurrence frequencies of sequential items and the transition probabilities \cite{maheu_rational_2022, SAFFRAN199927,yang_universal_2004}. For example, in artificial grammar learning, participants learn grammatical strings generated from a finite state language \citep{chomsky.miller1958} specified by a transition matrix defined on a set of artificial vocabulary. After exposure to the sequence, participants can judge a set of test strings' consistency with the language with above-chance accuracy \citep{Dulany1984}. Models that learn the associative transition probabilities between the sequential units can reproduce participants' performance in this task \citep{gomez_artificial_1999, SAFFRAN1996, gomez_variability_2002}. 

% [x] chunking models
On top of first-order transition statistics, people also tend to segment a sequence into disjunctive patterns. Studies have shown that upon hearing continuous input streams generated by an artificial language, children segmented the input stream into discrete recurring parts. This phenomenon was first explained by PARSER \citep{PERRUCHET1998246}, a model that parses a sequence by disjunctive chunks, whose size is randomly sampled and where each chunk is associated with a weight that increments with observational frequency and decrements via forgetting. PARSER can produce artificial language stream segmentations of continuous input streams without episodic cues such as pauses.  Other models that acquire repeated patterns from sequences as chunks, such as CCN (competitive chunker) \cite{anderson1990}, are symbolic models that learn chunks from already-encountered items and construct a hierarchy of chunks as subjects remember sentences. Such models have been shown to replicate grammaticality judgments from sequences with distinct hierarchy levels (e.g., word level vs. phrase level).

Going beyond seeing chunking and statistical learning as heuristics or tendencies of human behavior, we take a normative approach and hypothesize that learning statistics and chunks are rational strategies adapted by a learning agent to discover underlying structures in sequences with embedded hierarchy. 


\subsection{Parsing a sequence one chunk at a time}
% set up sequences 
% [x] parsing
Observation sequences are made up of discrete, integer-valued, size-one elementary observational units coming from an atomic alphabet set $\mathbb{A}$. The sequence $S$ is parsed one chunk at a time and segmented into disjoint units. An example of such a sequence could be $010021002112000...$, and so forth. The agent learns chunks from the sequences and stores them in a belief set $\mathbb{B}$. When the model learns the following chunks $\{0,1,21,211,12,2112\}$, the sequence can be partitioned in the following way:  \underline{0} \underline{1} \underline{0} \underline{0} \underline{21} \underline{0} \underline{0} \underline{2112} \underline{0} \underline{0} \underline{0}.

The agent assumes that a sequence is generated from samples of independently occurring chunks with the probability of $P_\mathbb{B}(c)$ evaluated on the belief set $\mathbb{B}$. The probability of observing a sequence $S$ of parsed chunks $S = (c_1,c_2,..., c_{N})$ can be denoted as $P(S) =P(c_1,c_2,..., c_{N}) = \prod_{c_i \in \mathbb{B}} P_{\mathbb{B}}(c_i)$. Chunks as perceiving units serve as independent factors that disentangle observations in the sequence. %From this formulation, questions can be asked, such as what chunks in the belief set that make the sequence parsing probability higher. 

\subsection{Learning associations}
% update marginal and transition probabilities
Upon parsing, the model updates the observational and transition frequencies between subsequently parsed chunks. The agent learns chunks and stores them in the belief set $\mathbb{B}$. We assume that the learning agent can keep track of the marginal parsing frequency $\mathbb{M}(c_i)$ for each chunk $c_i$ in $\mathbb{B}$, a vector with size $|\mathbb{B}|$ and the transition frequency $\mathbb{T}$ between chunk $c_i$ followed by chunk $c_j$. 
Along with each parse $t$, the transition counts between the previous $c_L$ and next chunks $c_R$ are recursively updated: $T_{ij}(t+1) = T_{ij}(t) + [i = c_L][j = c_{R}]$, where
$[ \cdot ] = 1$ if the argument is true and 0 otherwise, and along with the identification frequency of each parsed chunk $M_{i}(t+1) = M_{i}(t) + [i = c]$. When modeling human behavior, entries of $M$ and $T$ multiply with a memory decay parameter $0 \leq \theta \leq 1$ per parsing step. 

\section{Bridging from the simple to the complex }
We propose that learning sequence statistics - when combined with learning chunks - enable the learning agent to recursively compose more complex representations by reusing the previously learned ones.
This allows a learning agent without any primitive assumptions about the sequence to adapt and grow representations adapting to the nested hierarchies in the sequences. It allows a model with no chunk knowledge about the sequence to first parse sequences in the most parsimonious way on the granularity of atomic units. Cued by the statistical relationships between chunks in the belief set, it updates and enlarges the belief set, leading to better ways of factorizing the sequence via composing new chunks by updating the belief set. 

\section{Learning hierarchical chunks}
% [x] generative model for chunking
We generated sequences with a nested hierarchical structure to examine the effectiveness of chunks. 
A hierarchical graph generates the none-iid sequence of observations. Starting with an initial set of atomic chunks $\mathbb{A}_0$, at the i-th iteration, two chunks $c_{L}$, $c_{R}$ are randomly chosen from the current set of chunks $\mathbb{A}_i$ and are concatenated into a new chunk $c_{L} \oplus c_{R}$, augmenting $\mathbb{A}_i$ by one to $\mathbb{A}_{i+1}$. Meanwhile, an independent occurrence probability is assigned to each chunk under the constraint that the probability of occurrence for every new chunk $c_i$ in the construction process evaluated on the support set $\mathbb{A}_i$ carries the largest probability mass. Given such a graph hierarchy, a non-iid observational sequence is constructed by consecutively sampling chunks from the hierarchy with their corresponding probability under the constraint that no two chunks with a child chunk are sampled consecutively.


%Hierarchical structures have been proposed to arise from self-diversifying systems \citep{abler_particulate_1989, Sportiche2013, von1999humboldt}: a set of discrete units that form stable combinations with one another, whose synthesis `is not present in any of the associated constituents'. 
% [ ] model to learn chunks
Given that the observational sequence reflects the underlying structure in the generative model, we propose the hierarchical chunking model (HCM) to uncover the embedded hierarchical structure from sequences. Intuitively, recurring patterns will span several sequential units if a sequence contains an inherent hierarchical structure. When such patterns occur, observations between units within the pattern will be correlated. In this case, learning and storing the patterns in memory will help agents use fewer entities in memory to parse the sequence. HCM is initialized with an empty belief set $\mathbb{B}$, which is first populated by atomic sequential units as its entry. Chunks in the belief set are used to parse sequence. At every parsing step, the longest chunk in the belief set consistent with the upcoming sequence is chosen to explain the upcoming sequential observations. The end of the previous parse initiates the next parse.

% chunk merging mechanism 
HCM builds up and enlarges the belief set via a chunk proposal mechanism. Starting with the null hypothesis $\mathcal{H}_0$ that all consecutively parsed chunks $c_L$ and $c_R$ are statistically independent $P(c_L,c_R) = P(c_L)P(c_R)$. Entries in $\mathbb{M}$ and $\mathbb{T}$ are used to test the hypothesis that consecutive chunk parses have a correlated consecutive parse within the sequence via a $\chi^2$-independence test. If there are correlations between the chunk pairs below the significance level of $p = 0.05$ with a $\chi^2$ test, then the null hypothesis is rejected, and the pair is proposed to concatenate into a new chunk $c_L \oplus c_R$, which augments the belief set $\mathbb{B}$ by one. The chunk proposal mechanism prioritizes pairs that retain the largest joint probability. This process repeats until all of the chunks in the belief set pass an independence halting criterion via a $\chi^2$ test.

% , which measures if all of the chunks in the belief set used to parse the sequence significantly violate an independence testing criterion 

% why this model is hierarchical 
The previously learned chunks serve as building blocks for discovering more complex chunks in the hierarchy containing the simple chunk as their subpart. Patterns within a sequence as units simplify perceptual processing because the sequence can be perceived one chunk after another instead of one sequential unit at a time. 


% the interaction between belief set update and parsing, and different parsing choices. 
% different variations of HCM 
There are several versions of HCM adapted to different proposes. The rational chunk learning model proposes one chunk and expands the belief set upon the completion of parsing the sequence. The online version of the model proposes novel chunks on the go. To simulate behavioral data such as the reaction time needed to make a choice, the prediction of the next sequential item made by the model is translated to a higher starting point in a linear ballistic accumulator \cite{brownheathcote,donkin2011drawing}, more details can be found in the corresponding papers documenting the projects. 
%We prove in the SI section that restricted conditions in which the sub-objects constituting the object in the ground truth are parsed faithfully by the model as sub-chunks, then these sub-chunks will be eventually proposed to concatenate into one chunk. 

%Generic hierarchical pattern discovery algorithm that enables the rational discovery of structures with embedded hierarchies. 

%The representation learned by HCM can be described by a chunk hierarchy graph $\hat{\gG}$ as illustrated in example Figure~\ref{fig:hcm}d with vertex set being the learned chunks and edges pointing from chunk constituent to the concatenated chunks. As learning proceeds further into the training sequence, the new chunks acquired by HCM are gradually added as new vertices and edges to the chunk hierarchy graph. 

\section{From the simply abstract to the complexly abstract}
% maybe some motivation 
Apart from using the simple to construct the complex in concrete sequences, past work has also studied people's capability to learn abstract patterns \cite{Boole1854, Marcus2001TheAM,chomsky2014aspects}. Examples of such patterns include grammatical rules in language, symbolic description of physical laws, or motifs in music. We hypothesize that it is rational for intelligent agents to learn abstract concepts with sequences of data that contain a nested hierarchical structure with embedded categories.

% [x] generative model for abstraction learning
%We start from the premise that apart from the nested hierarchical structure that some parts are the components of other parts,  natural sequences contain and give rise to categories of objects that similarly interact with other objects \citep{abler_particulate_1989}. Uncovering stable recurring patterns and embedded categories helps agents to capture the relations and interactions of objects and components under observation. 
We propose a generative model of sequences with abstract and relational properties. The generative model also starts with a basic inventory, a set of atomic units $\mathbb{A}$ and expands the inventory by $d$ iterations. At each iteration, a novel pattern or category is created equi-probably and expands the inventory. A new category is created by pointing the category to a random selection of several existing patterns. A new pattern is created by concatenating a random set of pre-existing pattern or categories from the existing inventory. 

The observation sequence is produced by randomly sampling patterns from the inventory. If a pattern has categories inside it, one of the pattern associated with the category is chosen. This process is applied recursively until all categories randomly select their corresponding patterns. Ultimately, the observation sequence becomes a stream of discrete atomic units. 


\subsection{Learning model}
We propose an approximate recognition model that combines chunking with abstraction. Combining abstract entities as a part of chunking enables abstract patterns to also build up from the simple to the complex. We proposed a mechanism for coming up with abstractions and integrate this with the chunking model described before.

Abstraction is manifested in two ways: first, as finding common parts amongst the learned chunks for more efficient memory retrieval; and second, as grouping different perceptual items that interact in similar ways to form a \textit{variable}, so that a symbolic denotation of the variable may represent the occurrence of any chunk inside the category.

Abstraction as \textit{commonalities amongst memory items}  organizes the learned chunks into a parsing graph: the parent nodes are the biggest common prefix of the children nodes. The parsing graph effectively reduces the search steps as memory retrieval becomes navigating the parsing graph from the root until the deepest leaf consistent with the sequence, resembling a prefix tree structure \cite{Cunnings2018,dotlacil_parsing_2021, Anderson1974, Fredkin60} and reduces the search step in comparison to HCM. When a new chunk is introduced by concatenating existing chunks, an edge connects the left parent with the new chunk. This procedure allows the growth of the parsing graph with chunk addition, while preserving its structure. 

% The end of the previous parse initiates the next parse.

% HCM parses the sequence using the biggest chunks consistent with the upcoming sequence in the learned dictionary $\mathbb{C}$. This mechanism introduces computationally expense in the search process to locate the biggest explanatory chunk \cite{schreiber2023biologicallyplausible}. 

% many natural systems have hierachical structures in how their units interact. Learning about these structures is beneficial for compression and prediction.
%such as the constitution of molecules based on chemical elements, the constitution of biological units from genes, and the structure of human language


The second abstraction notion implemented in HVM is grouping different perceptual items that interact similarly to a \textit{variable} category.
The model proposes variable by grouping chunks that occur in a similar context ---- proceeded by the same chunk (common preadjacency) and succeeded by the same chunk (common adjacency). Given consistent parsing of subchunks as object combination components in the generative model, the true chunks that belong to the same category will necessarily appear in the preadjacency and postadjacency entries. HVM proposes variables based on significantly correlated chunks ($p \leq 0.05$) in the transition matrix consistent with this structure. Amongst the correlated consecutive chunk pairs, the model intersects every eligible transition column of post-adjacency and row of preadjacency to propose a new variable $v$ that entails a set of chunks $E(v) = \{c_1, c_2, ..., c_j\}$. Together, the common preceding chunk, in conjunction with the newly proposed variable, followed by the common succeeding chunk, will be proposed as a novel concatenated chunk $c_L \oplus v \oplus c_R$ to add to $\mathbb{C}$. An edge that connects  $c_L$ to the new chunk $c_L \oplus v \oplus c_R$ will be added to the parsing graph. This process introduces chunks with embedded variables. For example, consider the case that the sequence includes A-ABC, A-DC and  ABC-ED, DC-ED. This suggests that ABC and DC play similar roles relative to A (coming after) and ED (before). Therefore, ABC and ED can be proposed as a new variable V to represent the abstract property that captures the distinct entities. V entails chunks ABC and DC. The model identifies V if either ABC or DC is identified during parsing.

% Relating to our intuition that examples of a variable may include using an 'animal' to denote the occurrence of either a cat, a dog, or a squirrel. A variable entails several chunks and is parsed if any of its entailing chunks are identified. 

% During parsing, a chunk is consistent with the sequence when all of its included variables contain at least an entailing chunk consistent with the sequence.

% [ ] variations of this model as applied in different works 
Variations of this model have been adapted for different modeling proposes. When comparing models and studying the algorithmic characteristics, we used a rational version of the model that parses the sequence until completion per iteration and updates the dictionary. 
When modeling human behavior, the model updates chunks' transition and occurrence counts online. All the entries multiply with a memory decay parameter $0\leq \theta \leq 1$ for each parsing step. 



% This empowers the model to learn the complex from the simple both on an abstract and concrete level, allowing the model to understand patterns that are also complexly abstract.
% This allows the model to learn patterns that parse a sequence into chunks and form abstract patterns based on the previously learned chunks and the symbolic description of categories denoting chunks with similar interaction properties. In this way, the model can discover more complex and abstract patterns varying in degree and detail. 


% % statistical learning from the environment
% \cite{yang_universal_2004} Infants seem to keep track of statistical information such as the transition probabilities. TP is not enough to simulate word parts and boundaries for languages used in everyday speaking for children. They propose a model that competes grammar for their usage. 

% It was suggested by the previous work that the brain updates information both on determinstic sequence rules and continuous transition probabilisties \cite{maheu_rational_2022}. 

% % 
% \cite{maheu_rational_2022} test the hypothesis that humans treat statistical biases and determinstic rules as two distinct hypothesis. They designed a change point detection task where a sequence of binary tones switches from a random part to a statistical/rule part at a random point in the sequence unbeknownst to the participants. They ask participants to detect the change point of statistical regularity versus determinstic regularity that suddenly appear within a random sequence of binary observations. A well known feature of the auditory system is to detect a subpart of a repeating sequence forming a noticable temporal compound (AABABABABB). Participants need to report their detection and discrimination subjectively during the task. They argue that subjects treat statistics and rules as distinct hypothesis spaces rather than a continuum. No modulation of belief update for deterministic rules. Contrary to pure statistical biases, belief update of deterministic rules does not decrease with Shannon entropy of apparent first-order transition probabilities. Detection point of a determinstic pattern increases with sequence length and is usually abrupt. Whereas detection point of statistical biases is gradual. The more entropic the first-order transition probabilities are, the slower the detection process.  

% Our work can be related to several lines of previous research on chunking. Firstly, Servan-Schreiber and Anderson \cite{anderson1990} studied how chunking facilitates memory by examining subjects' memorization for artificially produced grammatical sentences. They proposed that a hierarchy of chunks forms as subjects remember sentences. They instructed subjects to memorize sentences chunked by distinct hierarchy levels (e.g., word level vs. phrase level) and examined subjects' judgment of grammaticality afterwards. Their result suggested that the hierarchy of chunks influenced participants' grammaticality judgments. Apart from that, subjects overtly chunked the training sentences even when presented in an unstructured way. These findings are similar to our current model which also predicts chunking to appear in unstructured data but does so via a trade-off between accuracy and speed.

==> content/glushoko_precis.tex <==
\section{Introduction}
% the importance of structured perception, and the open question
Immersed in chaotic and noisy sensory streams, we perceive a structured world. From learning stimulus-response pairings to grouping nearby visual parts, and from grammar acquisition to learning recurring sequential patterns, cognition irresistibly and swiftly breaks a high-dimensional sensory stream into familiar parts and gradually unveils their relations. Why do structures emerge, and how do they help us learn, generalize, and predict? What underlying computational principles give rise to this fundamental aspect of perception and intelligent behavior?

% sequence, chunking, normative 
A sensory stream --- simplified to an extreme --- is a one-dimensional discrete sequence. In the process of learning such sequences, we naturally segment them into familiar parts — a well-known phenomenon called chunking.
% contribution: relates chunking to resource rational trade-off between speed and accuracy 
In the first project, I investigated the factors that influence chunking behavior in a serial reaction time task. I showed that humans sensitively adapt to underlying chunks in sequences while exhibiting a resource-rational trade-off between speed and accuracy. 

% contribution: normative perspective
Taking a step further, I built models that capture the chunk learning process on a computational and algorithmic level. The model learns chunks and parses sequences one chunk after another. From a normative standpoint, I proposed that chunking can be a rational way for an intelligent agent to discover recurring patterns and nested hierarchies in sequences, and, in turn, factorize sequences more effectively. I showed that sequential chunks can be learned as readily accessible primitives, ready for reuse, transfer, composition, and mental stimulation. This consequently allows the model to build up a complex understanding of the world by seeing the new via composing the known. 
I demonstrated and generalized this model's ability to learn hierarchies in both single and multi-dimensional sequence domains, and showed its applicability as an unsupervised pattern discovery algorithm. 

The second part of the investigation dives from the concrete domain to the abstract domain. I taxonomized two abstract sequence motifs and studied their implications for sequence memory recall. Behavioral evidence suggests that humans readily exploit redundancies in patterns in an abstract space for more efficient memory compression while transferring these motifs to novel sequences. 

% contribution, connecting chunking with abstraction, 
Taking a step further, I propose a non-parametric hierarchical variable learning model that combines abstraction with chunking—abstracting those chunks that appear in similar contexts as variables while learning chunks also on a symbolic variable level --- gradually unearthing abstractions and discovering invariant patterns on a symbolic level. I demonstrate the algorithm's resemblance to human learning behavior and compare it with large language models. 

% a summary [improve]
Taken together, this thesis suggests that chunking and abstraction as simple computational principles give rise to structured knowledge acquisition in sequences with underlying hierarchical structure, from simple to complex, from concrete to abstract, enabling the recursive construction of the highly complex from the ground up. I demonstrated the models' resemblance to human behavior and their algorithmic applications to discover patterns.   

\section{Conclusion}
